Verification of Quantum Circuits through Discrete-Time Barrier Certificates

Current methods for verifying quantum computers are predominately based on interactive or automatic theorem provers. Considering that quantum computers are dynamical in nature, this paper employs and extends the concepts from the verification of dynamical systems to verify properties of quantum circuits. Our main contribution is to propose k-inductive barrier certificates over complex variables and show how to compute them using Hermitian Sum of Squares optimization. We apply this new technique to verify properties of different quantum circuits.

==> Images/barrier.tex <==
\begin{tikzpicture}[inner sep=6pt,scale=2]
        \node[rectangle, text width=5.5cm, align=center, draw] (realbc) {Barrier Certificate Constraints ($\in \mathbb{R}$)
        \\
        ${B(\init{x}) \leq 0}, {\forall \init{x} \in \init{\mathcal{X}}}$
        \\
        ${B(\unsafe{x}) > d}, {\forall \unsafe{x} \in \unsafe{\mathcal{X}}}$
        \\
        \dots
        };
        \node[rectangle, text width=4cm, align=center, right=of realbc, draw] (sos) {Barrier Generation (SOS)
        \\
        ${B(x) - \init{\lambda}(x) \init{g}(x)}$
        \\
        ${B(x) - d - \unsafe{\lambda}(x) \unsafe{g}(x)}$
        \\
        \dots
        };
        \draw[-latex] (realbc.east) -- (sos.west);
        \node[rectangle, text width=5.5cm, align=center, below=of realbc, draw] (complexbc) {Barrier Certificate Constraints ($\in \mathbb{C}$)
        \\
        ${B(z) = b(z, \overline{z})}$
        \\
        ${B(\init{z}) \leq 0}, {\forall \init{z} \in \init{\sysspace}}$
        \\
        ${B(\unsafe{z}) > d}, {\forall \unsafe{z} \in \unsafe{\sysspace}}$
        \\
        \dots
        };
        \node[rectangle, text width=4cm, align=center, right=of complexbc, draw] (hsos) {Barrier Generation (HSOS)
        \\
        ${B(z) - \init{\lambda}(z) \init{g}(z)}$
        \\
        ${B(z) - d - \unsafe{\lambda}(z) \unsafe{g}(z)}$
        \\
        \dots};
        \draw[-latex] (complexbc.east) -- (hsos.west);
\end{tikzpicture}

==> Images/grover.tex <==
\begin{quantikz}[slice style={blue}]
    & \gate{H}\slice{} & \gate[3][1.5cm]{O} & \gate[3][1.5cm]{D} & \gate[3][1.5cm]{O} & \gate[3][1.5cm]{D} & \\
    & \gate{H} & & & & & \rstick{\dots}\\
    & \gate{H} & & & & &
\end{quantikz}

==> Images/qcircuit.tex <==
\begin{quantikz}[slice style={blue}]
    & \gate[3][1cm]{U_0} & \push{\quad \dots \quad} & \gate[3][1cm]{U_{k-2}} & \gate[3][1cm]{U_{k-1}} & \qw{}\\
    & & \push{\quad \dots \quad} & & & \qw{} \\
    & & \push{\quad \dots \quad} & & & \qw{}
\end{quantikz}

==> Images/qcircuit2.tex <==
\begin{quantikz}[column sep=0.75cm]
    & \gate{H} \gategroup[3,steps=1,style={inner
sep=6pt}]{$U_0$}
    & \ctrl{2}\gategroup[3,steps=5,style={inner
sep=6pt}]{$U_1$} & \qw{} & \qw{} & \qw{} & \ctrl{2}
    & \gate{H}\gategroup[3,steps=1,style={inner
sep=6pt}]{$U_0$} & \qw{}\\
    & \gate{H}
    & \qw{} & \ctrl{1} & \qw{} & \ctrl{1} & \qw{}
    & \gate{H} & \qw{} \\
    & \gate{H}
    & \targ{} & \targ{} & \gate{Z} & \targ{} & \targ{}
    & \gate{H} & \qw{}
\end{quantikz}

==> Images/xz.tex <==
\begin{quantikz}
    & \gate{X} & \gate{Z} & \gate{X} & \gate{Z} & \\
    & \gate{X} & \gate{Z} & \gate{X} & \gate{Z} & \rstick{\dots} \\
    & \gate{X} & \gate{Z} & \gate{X} & \gate{Z} & 
\end{quantikz}

==> Sections/app_grover.tex <==

\section{Grover Example}
The unitary matrix for the oracle (with mark $m = 0$ and a 2 qubit system) is
\setlength{\arraycolsep}{3pt}
\begin{equation*}
    O = \begin{pmatrix}
        -1 & 0 & 0 & 0 \\
        0 & 1 & 0 & 0 \\
        0 & 0 & 1 & 0 \\
        0 & 0 & 0 & 1
    \end{pmatrix},
\end{equation*}
and the associated matrix for the diffusion step is
\begin{equation*}
    D = \frac{1}{2}
    \begin{pmatrix}
        -1 & 1 & 1 & 1 \\
        1 & -1 & 1 & 1 \\
        1 & 1 & -1 & 1 \\
        1 & 1 & 1 & -1
    \end{pmatrix}.
\end{equation*}

Then,
\begin{equation*}
    D.O = \frac{1}{2}
    \begin{pmatrix}
        1 & 1 & 1 & 1 \\
        -1 & -1 & 1 & 1 \\
        -1 & 1 & -1 & 1 \\
        -1 & 1 & 1 & -1
    \end{pmatrix},
\end{equation*}
and
\begin{equation*}
    O . D = \frac{1}{2}
    \begin{pmatrix}
        1 & -1 & -1 & -1 \\
        1 & -1 & 1 & 1 \\
        1 & 1 & -1 & 1 \\
        1 & 1 & 1 & -1
    \end{pmatrix}.
\end{equation*}

For m = 1:
\begin{equation*}
    D.O = \frac{1}{2}
    \begin{pmatrix}
        -1 & -1 & 1 & 1 \\
        1 & 1 & 1 & 1 \\
        1 & -1 & -1 & 1 \\
        1 & -1 & 1 & -1
    \end{pmatrix}
\end{equation*}

==> ccs.tex <==
\begin{CCSXML}
<ccs2012>
   <concept>
       <concept_id>10003752.10003753.10003758</concept_id>
       <concept_desc>Theory of computation~Quantum computation theory</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
   <concept>
       <concept_id>10003752.10003790.10002990</concept_id>
       <concept_desc>Theory of computation~Logic and verification</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
   <concept>
       <concept_id>10010520.10010553</concept_id>
       <concept_desc>Computer systems organization~Embedded and cyber-physical systems</concept_desc>
       <concept_significance>300</concept_significance>
       </concept>
 </ccs2012>
\end{CCSXML}

\ccsdesc[500]{Theory of computation~Quantum computation theory}
\ccsdesc[500]{Theory of computation~Logic and verification}
\ccsdesc[300]{Computer systems organization~Embedded and cyber-physical systems}
